Robustness to corruption in pre-trained Bayesian neural networks

We develop ShiftMatch, a new training-data-dependent likelihood for robustness to corruption in Bayesian neural networks (BNNs). ShiftMatch is inspired by the training-data-dependent "EmpCov" priors from Izmailov et al. (2021a), and efficiently matches test-time spatial correlations to those at training time. Critically, ShiftMatch is designed to leave the neural network's training time likelihood unchanged, allowing it to use publicly available samples from pre-trained BNNs. Using pre-trained HMC samples, ShiftMatch gives strong performance improvements on CIFAR-10-C, outperforms EmpCov priors (though ShiftMatch uses extra information from a minibatch of corrupted test points), and is perhaps the first Bayesian method capable of convincingly outperforming plain deep ensembles.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> neurips/meta.tex <==
We would like to thank the reviewers for their positive comments.
In response to reviewer comments, we have included a number of additional experiments, including experiments on ImageNet-C (Fig. 5), which continue to show the advantages of our method.

Perhaps surprisingly, our two negative reviewers had alot of good things to say about the paper:

EBSb:
> It is clear that this method is interesting to the Bayesian deep learning community, especially given the improvement in accuracy to common corruptions. The empirical evaluation is a strong point of the paper. The many datasets and ablations used for evaluation leave no doubt that the method is effective at boosting the accuracy of neural networks.
fgix:
> ShiftMatch makes intuitive sense by whitening the noise of the test distribution and redistributing it according to the distribution of the training set.
> ShiftMatch can be applied to large pretrained models.
> The performance is strong.

Their central concerns appear to be easily fixable points about the manuscript text, rather than substantive issues about the method or experiments.

EBSb raised an issue surrounding confusion over which types of OOD input we sought to address.  Our paper was only about corruptions (as in CIFAR-10C and ImageNet-C), not e.g. adversarial inputs or OOD detection.  We have considerably altered the text to correct this confusion, and would additionally request to change the title to "Robustness to corruption in pre-trained (Bayesian) neural networks".

fgix noted that we had not emphasised that EmpCov priors are in a slightly different and harder setting, because our method uses a minibatch of corrupted test data, while EmpCov priors did not.  We have therefore updated the abstract, figure captions, main text and conclusion to emphasise this point.  And we would note that our comparisons against test-time batchnorm are fair, because test-time batchnorm also uses a minibatch of corrupted test data.

==> neurips/response.tex <==
> I think the first part of this response may have misunderstood my point. I never meant to imply that you were in competition with [1]. I meant that the comparisons in figures 1 and 3 draw comparisons to non-transductive models so the ShiftMatch results in those figures has the benefit of seeing and learning from more data than the other models.

We agree that ShiftMatch is in a slightly different setting, in that at test-time it requires a **minibatch** of corrupted inputs (in order to estimate the statistics) while other methods allow for a single sample as the input. 
As such (and as discussed in the original response), we added a discussion of this point to the:
* the abstract
* captions for figures 1, 3 and 5
* the conclusion
* various other places in the main text

Please let us know if you'd like any further revisions to further emphasise this point!

In response to your comments, we did consider deleting Figures 1 + 3 to avoid these comparisons between methods in slightly different settings.  This is certainly something we could do, given that we'd still have comparisons against test-time batchnorm, which are fair.  But ultimately, we lent towards keeping Figures 1 + 3 due to two main factors:
1. These are the only methods for corruption robustness in the Bayesian setting, so it is important we compare them, even if they are in slightly different settings.
2. We spend most of the Introduction/Background discussing Izmailov et al. (2021), so we can hardly avoid making the comparison!  (Even if that comparison isn't quite fair, because, as is now noted in the abstract, captions and conclusions ShiftMatch requires a minibatch of corrupted inputs at test time, while the other methods work for a single corrupted input).

Please let us know if you have any further thoughts on how and whether to present these comparisons.

Additionally, we looked a bit more carefully at the terminology, and whether "transductive" learning is the appropriate label for our method.
Remember that our method is in exactly the same setting as test-time batchnorm.
We therefore looked at test-time batchnorm papers [1-3] to see how they describe their setting.
Those test-time batchnorm papers describe their setting as ``domain adaptation'' or ``corruption robustness'', but never mention transductive learning. In addition, in [1, 2], the authors explicitly differentiate test-time batchnorm with unsupervised domain adaptation (which is an example of transductive learning): 
> Domain adaptation usually has a predefined target domain with unlabeled dataset, while corruption robustness normally does not assume such a predefined corruption type ([1])

> A common theme in these approaches is that they assume access to a set of unlabeled samples from the test set at training time, whereas our focus is to apply an intervention at test time, after a model has been trained ([2])

Transductive learning appears to mirror the setting in that last quote, in that transductive learning allows access to the corrupted test inputs (but not labels) at _training time_.
In contrast, our method (and test-time batchnorm) are applied to neural networks that are pretrained using standard supervised learning protocols on uncorrupted training inputs only, without access to any (corrupted) test inputs. The only difference between our method and other methods in Fig.1 and Fig.3 is that, given a pretrained model, ShiftMatch (as well as test-time batchnorm) would perform an extra matching step to align the statistics of the corrupted minibatch to that of the clean data.


> If 1000 images are used in a test minibatch, which corruptions and which intensities are present in those 1000 images?

We use the standard setup for test-time batchnorm [1-3] where the test batch consists entirely of the same type of corruption and intensity. Importantly, we make extensive fair comparisons between our method and test-time batchnorm on both CIFAR-10-C (Fig 4) and ImageNet-C (Fig. 5).

[1] Benz, P., Zhang, C., Karjauv, A., and Kweon, I. S. Revisiting batch normalization for improving corruption robustness. In Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision, pp. 494–503, 2021.

[2] Nado, Zachary, et al. "Evaluating prediction-time batch normalization for robustness under covariate shift." arXiv preprint arXiv:2006.10963 (2020).

[3] Schneider, Steffen, et al. "Improving robustness against common corruptions by covariate shift adaptation." Advances in Neural Information Processing Systems 33 (2020): 11539-11551.

[4] Gammerman A, Vovk V, Vapnik V. Learning by transduction. UAI (1998)

[5] "A Discussion of Semi-Supervised Learning and Transduction," Chapter 25 of Semi-Supervised Learning, Olivier Chapelle, Bernhard Schölkopf and Alexander Zien, eds. (2006). MIT Press. A discussion of the difference between SSL and transduction.

==> neurips/response_archive.tex <==
Robustness to corruption vs OOD detection.

To reiterate the previous point, our 

Fourth, we have added evaluations of the ShiftMatch's performance on OOD detection tasks (CIFAR-10 vs SVHN and CIFAR-10 vs CIFAR-100), and the results are presented in Appendix C. 
BNNs with and without ShiftMatch are better than other methods (SGD and deep ensembles) on all tasks and metrics.
However, the comparison between HMC and ShiftMatch is inconclusive, with HMC winning on CIFAR-10 vs CIFAR-100, and ShiftMatch winning on CIFAR-10 vs SVHN.
Thus, the strongest conclusion we can reach is that we as yet have no evidence that ShiftMatch hurts OOD detection performance.
This is expected: ShiftMatch is designed to improve robustness to corruption, _not_ to improve OOD detection.

As is suggested by R2, we added a comparison between different combination in Appendx, Fig. 8.

==> reviews.tex <==
Reviewer 

> EmpCov seems to transform only the input layers, but ShiftMatch seems to be applied for all the intermediate layers. Can you comment on this difference? For instance, would the performance of ShiftMatch be degraded if only applied to the input layers?

We did these ablations in Appendix D in the original manuscript.  In particular, see Figure 7, where the second column "ShiftMatch (input only)" is ShiftMatch applied only to the input layer.  We see that applying ShiftMatch at all layers roughly doubles the benefit of applying ShiftMatch only at the input layers, and that this grows at higher intensities.

Note that applying EmpCov priors at multiple layers is very difficult, because the prior over weights at an intermediate layer depends on the inputs to that layer, and those inputs in turn depend on earlier weights.  This difficulty is likely why they did not use multi-layer EmpCov priors in Izmailov et al. (2021a).

> In page 7, the paper explains the reason why ShiftMatch performs poorly for "Translate" corruption. It seems that ShiftMatch also underperforms baselines for "Scale", and slightly underperforms deep ensembles for "Gauss blur". The latter is quite disappointing since section 4.6 explains how ShiftMatch can "perfectly" removes stationary linear corruptions. Can you comment on this?

In Fig. 3 on page 7, it is ``glass blur'', _not_ ``Gauss blur''.  Looking at the original paper (Mu & Gilmer 2019) these are indeed very different from a Gaussian blur.

> I don't expect the size of the training data to stably estimate the statistics to be large. Having said that, one could think of a bagging-like procedure where multiple subsets of training data are sampled, corresponding statistics are computed, and multiple predictions are computed from the multiple statistics to be ensembled. This may make the interpretation of the data-dependent likelihood more cumbersome, but may enhance the robustness of the method.

Agreed!  We will investigate these possibilities in future work!



Reviewer BEej

The key claim in Sec. 4.1 is that models with EmpCov priors and ShiftEmpCov likelihoods have equivalent behaviour, because the distribution of the outputs of a layer with an EmpCov prior and a ShiftEmpCov likelihood are the same.

To formalise this notion of equivalence, we need to look at a function-space viewpoint, which works with the distribution over the logits output by the full network, $F$.
The function-space viewpoint is obtained by marginalising out the weights [REFs].
While explicit calculations are difficult in this viewpoint, it is very useful for establishing theoretical properties.
In particular, as the class labels are independent of the inputs, $X$, conditioned on the logits, $F$, we can write the graphical model as,
\begin{align}
  X \rightarrow F \rightarrow y.
\end{align}
Here, we combine the training and test points, $X=(X_{\rm train}, X_{\rm test})$, $F=(F_{\rm train}, F_{\rm test})$ and $y=(y_{\rm train}, y_{\rm test})$.
The prior over logits, $P(F| X)$ is the same in both EmpCov and ShiftEmpCov viewpoints, because the prior distribution of the outputs of each layer is the same.
Likewise, the softmax likelihood $P(y| F)$ is again the same in both EmpCov and ShiftEmpCov viewpoints.
As the priors are exactly equivalent under the two viewpoints, the posteriors over all quantities here must also be equivalent, and we can go further and explicitly write out the equivalent posteriors.
In particular, we want the posterior over train and test logits, $F$, conditioned on training labels, $y_{\rm train}$,
\begin{align}
  P(F| X, y_{\rm train}) &\propto P(y_{\rm train}| F_{\rm train}) P(F|X).
\end{align}
Remember that $F = (F_{\rm train}, F_{\rm test})$ and $X=(X_{\rm train}, X_{\rm test})$.
Again, this posterior is the same for the EmpCov and ShiftEmpCov viewpoints, because the prior, $P(F|X)$, is the same, and because the softmax likelihood, $P(y_{\rm train}| F_{\rm train})$ is the same.
From the posterior over logits, we can obtain the predictive distribution over test labels,
\begin{align}
  P(y_{\rm test}| X, y_{\rm train}) = \int dF P(y_{\rm test}| F) P(F|X, y_{\rm train})
\end{align}
and this is again equivalent because the posterior over logits is equivalent, and the softmax likelihood is equivalent.  We have included this in a new Appendix (Appendix B).

> I wonder if it will work well even if half of images are corruption-free and the other half are corrupted by intensity 5. Considering the idea of proposed method, I'm worried that it works well only for one unified corruption intensity.

Thanks for the suggestion! We did just this, and have added the results to Appendix I.  
For all methods tested (SGD, deep ensembles and HMC), we still see improvements for ShiftMatch over test-time batchnorm and the plain method, except for the SGD log-likelihood.
These improvements are still considerable, but are less spectacular than those in Fig. 4.

> Is it much more effective to match the distribution in all layers than to match only the distribution of input data? I wonder what it means to consider all the layers.

We did these ablations in Appendix D in the original manuscript.  In particular, see Figure 7, where the second column "ShiftMatch (input only)" is ShiftMatch applied only to the input layer.  We see that applying ShiftMatch at all layers roughly doubles the benefit of applying ShiftMatch only at the input layers, and that this grows at higher intensities.

> It would have been nice to measure the "Expected Calibration Error", which is commonly used to evaluate Bayesian models on classification problem.

We have added these results in Appendix H, Fig 10. 
Broadly, SGD has very poor accuracy and ECE, while ShiftMatch performs best in terms of accuracy, and deep ensembles performs best in terms of accuracy.
We could understand these results as ShiftMatch trading a bit of ECE for alot of accuracy (see Fig. 10 right).
However, comparing ECE is difficult when accuracy differs so dramatically (e.g. for corruption intensity 5) (see [1] for further details).
As one example, remember that ECE bins the models confidence (e.g. in the range 0.5--0.6), and asks whether the model's probability of being correct is close to the confidence (in this case, the probability of being correct should be about 0.55).
When the model is more accurate, more of its probabilities will be close to 0 or close to 1, meaning that there will be fewer samples in the intermediate bins (e.g. see Figure 3 in [2]). 
Having fewer samples in the intermediate bins implies that there will be larger errors in the calibration curves just due to finite samples, and larger errors in the calibration curve of course means a higher ECE. 
This is one example where changes in the ECE may occur not due to changes in the model's actual calibration, but due to finite sampling errors.

In addition, we have results on uncertainty-based OOD detection in Table 1, showing that ShiftMatch does not seem to have a detrimental effect on OOD detection.


[1] Nixon J, Dusenberry MW, Zhang L, Jerfel G, Tran D. Measuring Calibration in Deep Learning. CVPR Workshops (2019).
[2] Garriga-Alonso, A., Rasmussen, C.E. and Aitchison, L., 2018. Deep convolutional networks as shallow gaussian processes. ICLR (2019).


Reviewer NoHk



> Experiments are missing comparison with other methods that deal with corruptions or covariate shift. The only baseline that directly addresses the same problem is EmpCov, but there are other works, e.g., Trinh et al. 2022. Tackling covariate shift with node-based Bayesian neural networks. ICML.

Thanks for this reference!  We have added it to the related work, and we will investigate adding this method to our plots. As far as we can see, their performance is quite a bit worse than our results.  For instance, in our Fig. 1, we have an accuracy of just over 80\% for ShiftMatch for the highest intensity corruptions on CIFAR-10-C.  In contrast, in Trinh et al. Fig. 10, they have accuracies going up to only around 65\% for the highest intensity corruptions. Further, our Fig. 1 shows big differences from ShiftMatch to strong baselines such as plain deep ensembles.  In contrast, Trinh et al. seems to show only small differences (at least in accuracy) between their method and their baselines.

In general, finding comparable baselines is quite hard, as we are in a very restrictive setting:
* our approach does not modify network training (Trinh et al. does propose a new variational objective).
* our approach is cheap at test-time, and is therefore applicable to large ensembles (unlike e.g. TENT that requires some gradient steps at test-time).
* ideally, baselines would be in the Bayesian setting with a valid likelihood

But of course we are open to any other suggestions!

> Test time runtime discussion is missing. The paper rightly so emphasises that training time is unaffected by ShiftMatch, but how slower does the test time become with ShiftMatch? There is a brief mentioning of runtime for spatial batchnorm (a potential implementation of ShiftMatch).

For the CIFAR-10 experiments, given a test batch of 10,000 samples, it takes 1.15s for one forward propagation without ShiftMatch and 1.84s with ShiftMatch.  Given the large potential improvements in accuracy, this cost is likely to be worthwhile in many application domains.

[1] Gal, Yarin, and Zoubin Ghahramani. "Dropout as a bayesian approximation: Representing model uncertainty in deep learning." international conference on machine learning. PMLR, 2016.

[2] Kingma, Durk P., Tim Salimans, and Max Welling. "Variational dropout and the local reparameterization trick." Advances in neural information processing systems 28 (2015).

### Other comments/suggestions (these don’t impact the score):

> Acronyms such as SGD and FRN and HMC are not defined in the text

Fixed

> Introduction, first paragraph. "images" – the text prior to that was not limited to images only

Fixed

> Figure 1 caption. "HMC, SGD, Deep Ensemble, SGLD, mean-field VI" - missing references

Fixed

> After eq.(3): "C is the number of features, ... from the inputs to a single feature in the first hidden layer". If I understand correctly C is the number of features in the input layer, which should be emphasised to distinguish from that single feature in the first hidden layer

Fixed (we now use $M$ for the number of features, and $C$ for the number of channels).

> Page 3, last paragraph. “including for robustness” – weird wording

Fixed

> Page 3, last paragraph. “C is the number of channels” – first, channels were not properly introduced here and C has been used before to denote the number of features

We now use $M$ for the number of features, and introduced channel/height/width first

> Around eq. (12)-(13). It is probably worth mentioning that priors are assumed to be the same in the “standard BNN” and in the BNN with ShiftMatch

fixed

> Eq. (14). C has been used already to denote the number of features and the number of channels

Fixed: changed the matrix $C$ to the matrix $S$.

> Figure 3 caption. Ensembles are not mentioned

Fixed.

> Page 7, bottom. It would be interesting to see a discussion on why on some corruptions the ensemble works better and on some worse than ShiftMatch.

As expected, ShiftMatch performs well when the corruption changes the "texture" of the image, e.g. in brightness, fog, zigzag or canny edges.  At the same time, there are two examples where ShiftMatch performs particularly badly: scale and translate.  Before going on, it is worth remembering that the usual way to deal with scale and translation corruptions is data-augmentation, which was not used in this training procedure, as we were mirroring Izmailov et al. (2021).  On scale and translate, it seems here that ShiftMatch is doing badly, rather than ensembles is doing well, as for rotate, ensembles is the same as HMC and EmpCov, while for translate, ensembles is slightly worse than the other two.  We would speculate that the reason is that both translate and scale are highly non-stationary (i.e. they cannot be corrected by modifying the power spectrum of the image), so we would not expect ShiftMatch to perform well on these images.  At the same time, we would speculate that these translations are changing the spatial structure of the images, and ShiftMatch's attempts at correcting these spatial shifts turns out to be detrimental.

> Figure 5 caption. ImageNet-C is missing a reference.

Fixed.

> Appendix B. Which data has been used here? “Tab.3 gives performance differences with and without ShiftMatch” – was it meant to be “batchnorm” here?

Fixed.

> Eq. (10) "." -> ","

Fixed

> Sec. 4.6. First sentence. "ShiftMatch retains all useful the theoretical properties" -> "ShiftMatch retains all the useful theoretical properties"

> Conclusion. Second sentence. "Shiftmatch" -> "ShiftMatch"

Fixed.

> Appendix A. last line. S -> Sigma

Fixed.


